RoSI: Recovering 3D Shape Interiors from Few Articulation Images

The dominant majority of 3D models that appear in gaming, VR/AR, and those we use to train geometric deep learning algorithms are incomplete, since they are modeled as surface meshes and missing their interior structures. We present a learning framework to recover the shape interiors (RoSI) of existing 3D models with only their exteriors from multi-view and multi-articulation images. Given a set of RGB images that capture a target 3D object in different articulated poses, possibly from only few views, our method infers the interior planes that are observable in the input images. Our neural architecture is trained in a category-agnostic manner and it consists of a motion-aware multi-view analysis phase including pose, depth, and motion estimations, followed by interior plane detection in images and 3D space, and finally multi-view plane fusion. In addition, our method also predicts part articulations and is able to realize and even extrapolate the captured motions on the target 3D object. We evaluate our method by quantitative and qualitative comparisons to baselines and alternative solutions, as well as testing on untrained object categories and real image inputs to assess its generalization capabilities.

==> 7_dataset.tex <==
\section{Dataset}
\label{sec:dataset}

We use the PartNet-Mobility dataset \cite{xiang2020sapien} for all our experiments, which is a part-segmented 3D shape dataset with ground-truth annotation on part motions. We consider 9 categories of objects: Storage, Bin, Fridge, Microwave, Washer, Dishwasher, Oven, Safe and Box. When moveable parts in shapes belonging to these categories are articulated, they reveal planar interior regions, which is the reason such categories were selected to work with (as opposed to categories such as Stapler, Pliers, Scissors, USB etc.). 

Since no annotations for object interiors are available, we identify interior regions by ray-casting. We shoot rays from a source and find faces on the part-segmented 3D object mesh the rays intersect with. An articulated 3D model reveals new intersecting faces that are not otherwise present when using the rest-state 3D model. These new faces are then said to correspond to the object's interior. This setting allows us to obtain ground-truth depth, camera pose, binary articulated part masks (in 2D) and binary interior region masks (in 2D). To obtain ground-truth plane parameters (in 3D) for the interior planes, we use multi-plane RANSAC algorithm \cite{fischler1981random} on the 3D point cloud of 2D interior masks. Images are rendered using the Mitsuba renderer \cite{jakob2022mitsuba3} at $256^{2}$ resolution. We assume a consistent camera intrinsic matrix for all images. More details can be found in the \agp{supplementary}.
In total, after data filtering based on incorrect motion annotations and parts with few faces, we consider a total of 350 shapes, with a 75-25 train-test split.

